Graph-Based Logic and Sketches II: Finite-Product Categories and Equational Logic (Preliminary Report)

It is shown that the proof theory for sketches and forms provided in Part I of this paper (see http://www.cwru.edu/1/class/mans/math/pub/wells) is strong enough to produce all the theorems of the entailment system for multisorted equational logic provided in Goguen and Meseguer's article ``Completeness of many-sorted equational logic'' (Technical Report CSL-135, SRI International Computer Science Laboratory, 333 Ravenswood Ave., Menlo Park, CA 94025, USA, 1982).

==> arthead.tex <==
\typeout{This is arthead.tex 22 October 1996}


\makeatletter

\hyphenation{Grothen-dieck equiva-lent
equiva-lence equiva-lents work-space man-u-script
codo-main pre-print pre-requi-site requi-site
non-empty Dia-gram-mes Ca-hiers endo-func-tor
single-ton Ehres-mann neces-sary
inte-ger inte-gers  Theo-rem Propo-si-tion Lem-ma Defi-ni-tion
epi-morph-ism iso-morph-ism endo-morph-ism auto-morph-ism
mono-morph-ism mono-morph-isms
epi-morph-isms iso-morph-isms endo-morph-isms auto-morph-isms
Archi-me-dean
homo-morph-isms iso-morphic
homo-morph-ism over-view
Grund-lehren Wis-sen-schaf-ten mon-oid
Wil-liam Ten-nes-see topo-lo-gie Knox-ville to-poses
man-u-script man-u-scripts ap-pen-dix data-base data-bases
ana-lyze ana-lyzes ana-lyzed ana-lyzing dis-trib-ute dis-trib-uted
dis-trib-utor dis-trib-utors be-hav-iour be-hav-iours pre-am-ble
pre-am-bles post-am-ble post-am-bles flocci-nauci-nihili-pili-fi-ca-tion
fest-schrift Sprach-wissen-schaft skinny-dip skinny-dip-ping
sphyg-mo-mano-meter medi-ocre oeuvres demi-semi-quaver hemi-demi-semi-quaver
semi-quaver praise-worthy
param-e-trised polyg-on-i-sa-tion kwash-i-or-kor
poly-sty-rene poly-sor-bate poly-un-sat-u-rate poly-un-sat-u-rated
ein-stein-ium men-del-ev-ium
pseudo-in-tel-lec-tual re-ed-u-cate re-ed-u-cated re-ed-u-ca-tion
re-ed-u-cat-ing re-ed-u-cates re-en-list re-en-listed re-en-lists
re-en-list-ing re-en-list-ment veri-si-mil-i-tude arc-tan-gent
arc-co-sine arc-co-tan-gent arc-co-se-cant Liech-ten-stein
Der-zhan-ski Chiang
anom-a-ly anom-a-lies an-tin-o-my an-tin-o-mies band-leader
band-leaders bor-no-log-i-cal Brown-ian buzz-word buzz-words cart-wheel
cart-wheels cho-les-teric data-path data-paths demos Dijk-stra
electro-mechan-i-cal electro-mechano-acoustic equi-vari-ance equi-vari-ant
Euler-ian fermi-ons flow-chart flow-charts Gauss-ian geo-met-ric Greifs-wald
Grothen-dieck Grund-leh-ren Hamil-ton-ian Her-mit-ian in-fra-struc-ture
infra-struc-ture jerem-i-ads Kadomt-sev Le-gendre Lip-schitz Lip-schitz-ian
macro-eco-nomic macro-eco-nomics Markov-ian meta-lan-guage meta-lan-guage
micro-eco-nomic micro-eco-nomics micro-fiche mod-el-ling mono-en-er-getic
mono-pole mono-strofic mul-ti-plic-able mul-ti-plic-ably neo-fields
Noether-ian non-emer-gency non-equi-vari-ance non-euclid-ean non-smooth
param-e-trized para-mil-i-tary poly-ene polyg-on-i-za-tion
pseu-do-dif-fer-en-tial pseu-do-fi-nite pseu-do-fi-nite-ly pseu-do-forces
pseu-do-word pseu-do-words qua-drat-ic qua-drat-ics qua-si-equiv-a-lence
qua-si-hy-po-nor-mal qua-si-smooth qua-si-sta-tion-ary Rie-mann-ian
sched-ul-ing Schwarz-schild semi-def-in-ite semi-ho-mo-thet-ies
ser-vo-mech-anism set-up sole-noid sole-noids spher-oid spher-oids
sto-chas-tic sub-scrib-er sub-scrib-ers sum-ma-ble ther-mo-elas-tic
time-stamp time-stamps ver-all-ge-mein-erte Wahr-schein-lich-keits-the-o-rie
wave-guide}





\message{new fonts,}
%% \input myfonts
\long\def\put(#1,#2)#3{\@killglue\raise#2\unitlength\hbox to \z@{\kern
#1\unitlength #3\hss}\message{.}\ignorespaces}

% \def\thebibliography#1{\section*{References\@mkboth
%  {REFERENCES}{REFERENCES}}\list
%  {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
%  \advance\leftmargin\labelsep
%  \usecounter{enumi}}
%  \def\newblock{\hskip .11em plus .33em minus .07em}
%  \sloppy\clubpenalty4000\widowpenalty4000
%  \sfcode`\.=1000\relax}
% \let\endthebibliography=\endlist

\def\doubleslash{//\penalty\exhyphenpenalty}
\def\pd{.\penalty\exhyphenpenalty}


\mathchardef\gt="313E %relation
\mathchardef\lt="313C %relation
\mathchardef\lte="0214 %\leq, with class of ordinary char
\mathcode`<="4268 %left delimiter
\mathcode`>="5269 %right delimiter
\mathcode`:="203A
\mathchardef\bq="4060
\mathchardef\eq="5027
\mathchardef\lsb="005B %left square bracket
\mathchardef\rsb="005D
%\def\ap{\kern 1pt\raise 1.4ex \hbox{$\mathchar"37A$}\kern 1pt}
\def\[{[\kern-1.2pt [}
\def\]{]\kern-1.2pt ]}
\def\R{{\bbold R}}
\def\Z{{\bbold Z}}
\def\Q{{\bbold Q}}
\def\N{{\bbold N}}






\message{changes in parameters,}

\lefthyphenmin=3

\message{constructed symbols,}
\def\epi{\mathrel{\mathchar"221\mkern -12mu\mathchar"221}}
\def\leftepi{\mathrel{\mathchar"220\mkern -12mu\mathchar"220}}
\def\mon{\mathrel{\m@th\hbox to 14.6pt{\lasy\char'51\kern-2pt$\arrext$\hss
$\mathord\rightarrow$}}} % width of \epi
\def\leftmono{\mathrel{\m@th\hbox to
14.6pt{$\mathord\leftarrow$\hss$\arrext$\kern-2pt\lasy\char'50%
}}} % width of \epi

\mathchardef\arrext="0200       % amr minus for arrow extension (see \into)
\def\addtotextheight#1{\advance\textheight by #1 \advance\@colht by #1
   \advance\@colroom by @1 \advance\vsize by #1}
\def\relstack#1#2#3{\mathrel{\mathop{#1}\limits^{%
    \textstyle#2}\limits_{\textstyle#3}}}
% \def\pf{\par\addvspace{\medskipamount}\noindent Proof.\emskip}
\def\Box{\vbox{\hrule\hbox{\vrule\kern.5ex
   \vbox{\kern1ex}\kern.5ex\vrule}\hrule}}
\newcommand\epf{~\hfill$\Box$\par\addvspace{\medskipamount}}

\newmuskip\tinymuskip
\tinymuskip=1.3mu
\renewcommand{\o}%
{\raise.2ex\hbox{$\scriptstyle\mskip\tinymuskip\circ\mskip\tinymuskip$}}

\newcommand{\op}{^{\rm op}}

\message{renamed symbols,}

\newcommand{\ba}{\mapsto}
% \newcommand{\e}{\exists}
\newcommand{\imp}{\Rightarrow}
\newcommand{\x}{\times}
\renewcommand{\a}{\forall}
\newcommand{\divides}{\mathbin{|}}

\message{command builders,}


\def\mathopdef#1{\expandafter\def\csname#1\endcsname{%
\mathop{\mbox{\rm #1}}\nolimits}}
\def\logopn#1{\expandafter\def\csname#1\endcsname{%
{\mathop{\mbox{\sf #1}}\nolimits}}}
\def\logord#1{\expandafter\def\csname#1\endcsname{%
{\mathord{\mbox{\sfi #1}}}}}
\def\mathopdef#1{\expandafter\def\csname#1\endcsname{{\mathop{#1\,}}}}
\def\mathbfdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\rm\bf #1}}}}
\def\mathrmdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\rm #1}}}}
\def\mathttdef#1{\expandafter\def\csname#1\endcsname{{\hbox{\tt #1}}}}
%% \def\mathcatname#1{\expandafter\def\csname#1\endcsname%
%% {\mbox{\catname #1}}}
\def\mathsketchname#1{\expandafter\def\csname#1\endcsname%
{\mbox{\sketchname #1}}}
\def\mathskd#1{\expandafter\def\csname#1\endcsname%
{\mbox{\skd #1}}}
\def\mathcatname#1{\expandafter\def\csname#1\endcsname{%
\mathop{\catname{#1\fake}}\nolimits}}


\message{new environments,}

% \input bezier.sty


% ENVIRONMENTS

\itemsep\smallskipamount\parsep0pt\topsep\medskipamount
\newcounter{lister}
\newcounter{underlister}

\newenvironment{reflist}{\vskip 4ex plus 1ex minus .2ex {\large\bf
\noindent References} \begin{trivlist}}{\end{trivlist}}

\newenvironment{romanlist}
{\begin{list}{(\roman{lister})}%
{\usecounter{lister}}}%begin text
{\end{list}}% end text
\newcommand{\romlist}{\begin{romanlist}}
\newcommand{\eromlist}{\end{romanlist}\noindent}

\newenvironment{alphalist}
{\begin{list}{\alph{lister})}%
{\usecounter{lister}}}%begin text
{\end{list}}% end text
\newcommand{\alist}{\begin{alphalist}}
\newcommand{\ealist}{\end{alphalist}\noindent}

\newenvironment{squishlist}
{\begin{list}{\alph{lister})}%
{\usecounter{lister}\parsep0pt\itemsep 0pt plus 2pt}}%begin text
{\end{list}}% end text
\newcommand{\sqlist}{\begin{squishlist}}
\newcommand{\esqlist}{\end{squishlist}\noindent}

\newenvironment{labeledlist}[1]
{\begin{list}{{\rm#1.\arabic{lister}}}{\usecounter{lister}
\settowidth{\labelwidth}{#1--1}
\leftmargin\labelwidth \advance\leftmargin by \labelsep
}}%begin text
{\end{list}}%

\newenvironment{underlist}[1]
{\begin{list}{{\rm#1--\arabic{underlister}}}{\usecounter{underlister}
\parsep0pt\settowidth{\labelwidth}{#1--1}
\leftmargin\labelwidth \advance\leftmargin by \labelsep
}}%begin text
{\end{list}}%


\message{new commands,}

\def\umlaut{\"}

\mathrmdef{dom}
\mathrmdef{cod}
\mathrmdef{id}
\mathrmdef{source}
\mathrmdef{target}
\mathrmdef{Hom}
\mathrmdef{ev}
\mathrmdef{Lim}
\mathrmdef{lim}
\mathrmdef{colim}

\def\darray{\begingroup\arraycolsep 2em
     \def\arraystretch{1.5}\array}
\def\enddarray{\endarray\endgroup}

% \def\a#1{\Asc_{#1}}
% \def\N#1{\mbox{\skd #1}}

\newcommand{\thm}{\specialsubsection{Theorem}\begingroup\em}
\newcommand{\thl}{\specialsubsection{Lemma}\begingroup\em}
\newcommand{\thp}{\specialsubsection{Proposition}\begingroup\em}
\newcommand{\thcv}{\specialsubsection{Convention}\begingroup\em}
\newcommand{\thc}{\specialsubsection{Corollary}\begingroup\em}
\newcommand{\defn}{\specialsubsection{Definition}\begingroup\rm}
\newcommand{\notat}{\specialsubsection{Notation}\begingroup\rm}
\newcommand{\rem}{\specialsubsection{Remark}\begingroup\rm}
\let\defd=\defn
\newcommand{\exam}{\specialsubsection{Example}\begingroup\rm}
\newcommand{\fp}{\specialsubsection{Fine points}\begingroup\rm}
\newcommand{\warning}{\specialsubsection{Warning}\begingroup\rm}
\newcommand{\meth}{\specialsubsection{Method}\begingroup\rm}
\newcommand{\spec}{\specialsubsection{Specification}\begingroup\rm}
\newcommand{\ethm}{\endgroup\par\pagebreak[2]\addvspace{\medskipamount}}
\let\eth=\ethm
\let\ethc=\ethm
\let\ethcv=\ethm
\let\ethp=\ethm
\let\eexam=\ethm
\let\ethl=\ethm
\let\edefn=\ethm
\let\enotat=\ethm
\let\erem=\ethm
\let\emeth=\ethm
\let\espec=\ethm
\let\ewarn=\ethm
\let\efp=\ethm
\def\pf{\specialsubsection*{Proof}}

\renewcommand{\sb}[2]{\{#1 \;\mid\;{#2}\}} % \sb was subscript

\def\bfdef{\bf}

\def\beqa{\begin{equation}\begin{array}{c}}
\def\eeqa{\end{array}\end{equation}\vskip 1ex\noindent}
% \def\itm{\item\hskip-1em}
\newcommand{\bc}{\begin{center}}
\def\beq{\begin{equation}}%for numbered equations and
\newcommand{\blist}[1]{\begin{labeledlist}{#1}}
\newcommand{\bp}{\begin{picture}}
\newcommand{\btable}{\begin{center}\begin{tabular}}
\newcommand{\ec}{\end{center}}
\def\eeq{\end{equation}}
\newcommand{\elist}{\end{labeledlist}}
\newcommand{\ep}{\end{picture}}
\newcommand{\etable}{\end{tabular}\end{center}}
%



%SPECIAL CHARACTERS

\def\|{\mathord{\mid}}

%\newcommand{\divides}{\mathbin{|}}
%\newcommand{\op}{^{\rm op}}
%\newcommand{\x}{\times}
%\renewcommand{\o}{\circ}%originally danish letter
%\newcommand{\ab}{\relax}
%\newcommand{\ov}{{\rm over}}
%\newcommand{\wrsym}{\mathop{\rm wr}\nolimits}
%\renewcommand{\wr}{\wrsym^}
%\renewcommand{\|}{\,\mid\,}

\newcommand{\0}{\emptyset}
\newcommand{\Cap}{\bigcap}
\newcommand{\Cup}{\bigcup}
\newcommand{\Deltop}{\mathbin{\Delta}}
\newcommand{\FALSE}{\mbox{\scriptsize FALSE}}
\newcommand{\Meet}{\bigwedge}
\newcommand{\Or}{\vee}%don't use "or" -- it's used in case
\newcommand{\Orrel}{\mathrel{\vee}}
\newcommand{\Orord}{\mathord{\vee}}
\newcommand{\Orbin}{\mathbin{\vee}}
\newcommand{\Rel}{\mathop{\rm Rel}\nolimits}
\newcommand{\Rplus}{\R^{\mathord{+}}}
\newcommand{\SQRT}{\mathop{\scriptsize SQRT}\nolimits}
\newcommand{\SQ}{\mathop{\scriptsize SQUARE}\nolimits}
\newcommand{\TRUE}{\mbox{\scriptsize TRUE}}
\newcommand{\ab}[1]{\left|#1\right|}
\newcommand{\alpharel}{\mathrel{\mbox{$\alpha$}}}
\newcommand{\alt}[2]{(\forall #1\mathord:#2)}
\newcommand{\al}[1]{(\forall #1)}
\newcommand{\all}{\forall}
\newcommand{\bra}{\{\}}
\newcommand{\ch}{\divides}%for choice in production
\newcommand{\cls}{\mbox{\rm cls}}
\newcommand{\comp}{^c}
\newcommand{\dash}{---}
\newcommand{\dollar}{\$}
\newcommand{\e}{\mathop{\rm e}\nolimits}
\newcommand{\ext}[2]{(\exists #1\mathord:#2)}
\newcommand{\ex}[1]{(\exists #1)}
\newcommand{\fs}[2]{\mbox{$\lsb#1\!\rightarrow\!#2\rsb$}}%function space
\newcommand{\gka}{\alpha}
\newcommand{\gkb}{\beta}
\newcommand{\gks}{\sigma}
\newcommand{\gkt}{\tau}
\newcommand{\gkg}{\gamma}
\newcommand{\gte}{\geq}
\newcommand{\gtbin}{\mathbin{\gt}}
\newcommand{\geqbin}{\mathbin{\geq}}
% \newcommand{\id}{\mathop{\rm id}\nolimits}
\def\implies{\Rightarrow}
\newcommand{\impliesord}{\mathord{\Rightarrow}}
\newcommand{\impliesbin}{\mathbin{\Rightarrow}}
\newcommand{\inord}{\mathord{\in}}
\newcommand{\inbin}{\mathbin{\in}}
\newcommand{\includedin}{\subseteq}
\newcommand{\inc}{\subseteq}
\newcommand{\intersect}{\cap}
\newcommand{\inverse}{^{-1}}
\newcommand{\iso}{\cong}
\newcommand{\join}{\vee}
\newcommand{\lab}{\left|}
\newcommand{\lsq}{\mbox{`}}%use in math mode to get single quote
\newcommand{\ltbin}{\mathbin{\lt}}
\newcommand{\leqbin}{\mathbin{\leq}}

\newcommand{\meet}{\wedge}
\newcommand{\mt}{\wedge}
\newcommand{\nn}{\hspace{-.5em}}
\newcommand{\n}{\mbox{\bf n}}
\newcommand{\pa}{\vfill\newpage}
\newcommand{\pws}{\Psc}
\newcommand{\rab}{\right|}
\newcommand{\res}{\divides}%for restriction
\newcommand{\rsq}{\mbox{'}}
\newcommand{\st}[1]{`#1\rsq}
\newcommand{\tl}{\leftarrow}
% \newcommand{\toleft}{\gets}
\newcommand{\uext}[2]{(\exists!\,#1\mathord:#2)}
\newcommand{\uex}[1]{(\exists!\,#1)}
\newcommand{\union}{\cup}
\newcommand{\us}{\Usc}%universal set
\newcommand{\uu}{\underline}
\newcommand{\yields}{\mbox{\large\ $\vdash$ }}
% \newcommand{\yields}{\mbox{\large$\vdash$}}

\renewcommand{\.}{\cdot}
\renewcommand{\Join}{\bigvee}%originally bowtie symbol
\renewcommand{\and}{\wedge}%Latex uses it for titles
\newcommand{\andord}{\mathord{\wedge}}
\newcommand{\andbin}{\mathbin{\wedge}}
\newcommand{\andrel}{\mathrel{\wedge}}
\renewcommand{\a}{\mbox{\bf a}}
\renewcommand{\equiv}{\Leftrightarrow}
\newcommand{\equivord}{\mathord{\Leftrightarrow}}
\newcommand{\equivbin}{\mathbin{\Leftrightarrow}}
\renewcommand{\i}{\cap}
\renewcommand{\lq}{``}
\renewcommand{\pmod}[1]{\allowbreak \mkern8mu ({\rm mod}\,\,#1)}
\renewcommand{\rq}{''}
\renewcommand{\u}{\cup}


\newcommand{\strinc}%
  {\mathrel{\mathop{\subset}%
  \hspace{-.75em}{\raisebox{-.75ex}{$\scriptstyle\neq$}}}}
\let\oldclude=\subset

\def\twodots{\mathinner{\ldotp\ldotp}}

\newcommand{\lst}[3]{#1_{#2},\ldots,#1_{#3}}
\newcommand{\lstsb}[3]{(#1_i\mid i\in #2\twodots #3)}

% \newcommand{\bfi}[1]{\index{#1}{\large\bf #1}}
% \newcommand{\bfi}[1]{\index{#1}{\bf #1}}
% \def\text#1{\:{\rm #1}\:}

\newcommand{\rinf}[2]{#1\;\yields\; #2}
\newcommand{\einf}[2]{\rinf{#1}{#2}\;\mbox{and}\;\rinf{#2}{#1}}
\newcommand{\fracl}[2]{\frac{\,#1\,}{#2}}
\newcommand{\sepp}{\hspace{1 em}}%
\newcommand{\law}[2]{$$#1\eqno{\mbox{#2}}$$}

% \newcommand{\cod}{\mathop{\rm cod}\nolimits}
% \newcommand{\dom}{\mathop{\rm dom}\nolimits}

\def\pbox(#1,#2)#3{\put(#1,#2){\mbox{#3}}}
%\def\putbox(#1,#2)#3{\put(#1,#2){\makebox(0,0){#3}}}
\def\relstack#1#2#3{\mathrel{\mathop{#1}\limits^{#2}\limits_{#3}}}
\newcount \repetitions
\def\repto#1{
\repetitions=0
\loop\ifnum\repetitions<#1
    \advance \repetitions by 1
    \relbar\joinrel
\repeat
\rightarrow
}
\def\reptwo#1{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\repto{#1}$}
\crcr \lower2pt\hbox{$\repto{#1}$}}}}}
\def\TO{\relbar\joinrel\relbar\joinrel\relbar\joinrel\rightarrow}
\def\TWOO{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\TO$}\crcr
    \lower2pt\hbox{$\TO$}}}}}
\def\TWO{\mathrel{\mathpalette\TWOO{}}}
\def\Tofro{\mathrel{\mathpalette\Toofro{}}}
\def\Toofro{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\longrightarrow$}
     \crcr \lower2pt\hbox{$\longleftarrow$}}}}}
\def\To{\longrightarrow}
\def\Twoo{\vcenter{\hbox{\ooalign{\raise3pt \hbox{$\longrightarrow$}
     \crcr \lower2pt\hbox{$\longrightarrow$}}}}}


\mathcatname{Set}
\mathcatname{Cat}
\mathcatname{Gr}
\mathcatname{Th}
\mathcatname{Mod}





\def\emph#1{{\em#1\/}}
\def\MAX{\mathbin{\rm max}}
\def\MIN{\mathbin{\rm min}}
\def\MOD{\mathbin{\rm mod}}
\def\DIV{\mathbin{\rm div}}
\def\TRUNC{\mathop{\rm trunc}\nolimits}
\def\FLOOR{\mathop{\rm floor}\nolimits}
\def\cons{\mathop{\rm cons}\nolimits}
\def\head{\mathop{\rm head}\nolimits}
\def\tail{\mathop{\rm tail}\nolimits}
\def\source{\mathop{\rm source}\nolimits}
\def\target{\mathop{\rm target}\nolimits}
\def\GCD{\mathop{\rm GCD}\nolimits}
\def\LCM{\mathop{\rm LCM}\nolimits}
\def\ABS{\mathop{\rm ABS}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}


%% The following makes small-print ragged-right marginal notes
% \def\@parboxrestore{\@arrayparboxrestore%
% \let\\=\@normalcr\raggedright}
\def\mpar#1{{%
\def\@parboxrestore{\@arrayparboxrestore\let\\=\@normalcr\raggedright}
\marginpar{{\footnotesize #1}}}}

\def\darray{\begingroup\arraycolsep 2em
     \def\arraystretch{1.5}\array}
\def\enddarray{\endarray\endgroup}



\message{Bibliography commands,}

\makeatletter
\let\@internalcite\cite
\def\cite{\def\citeauthoryear##1##2{##1, ##2}\@internalcite}
\def\shortcite{\def\citeauthoryear##1##2{##2}\@internalcite}
\def\@biblabel#1{\def\citeauthoryear##1##2{##1, ##2}[#1]\hfill}



\def\@citex[#1]#2{%
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\reset@font\bfseries ?}%
       \G@refundefinedtrue
       \@latex@warning
         {Citation `\@citeb' on page \thepage \space undefined}}%
       {\csname b@\@citeb\endcsname}}}{#1}}



\makeatother


% The following are for use when you don't use BibTeX.
% \def\book#1#2#3{{{\mbox{#1}}, }%
%    {{\bf #2. }}{#3.}\pagebreak[3]}
% \def\art#1#2#3{{{\mbox{#1}}, }%
%    {{\it #2. }}{#3.}\pagebreak[3]}
% \def\artc#1#2#3#4#5#6{{{\mbox{#1}}, }%
%    {{\it #2. }}{#3} {{\bf #4}} (#5), #6.\pagebreak[3]}
%
% \def\lnm#1{Lec\-ture Notes in Math\-e\-ma\-tics {\bf#1}}
% \def\lncs#1{Lec\-ture Notes in Com\-pu\-ter Sci\-ence {\bf#1}}
% \def\springer{Sprin\-ger-Ver\-lag }
% \def\cahiers#1{Cah\-iers de Topo\-lo\-gie et G\'e\-o\-m\'e\-trie
% Dif\-f\'e\-ren\-ti\-elle\ifnum#1>25 { Cat\-\'e\-go\-rique}\fi\ {\bf #1}}

\def\Frac#1#2{\frac{\displaystyle #1}{\displaystyle #2}}
\def\Rule#1#2{\Frac{\hspace{1em}#1\hspace{1em}}{#2}}
\makeatother

\makeatletter
\def\dmparms{
\normalsize
\@lowpenalty 151
\@medpenalty 651
\@highpenalty 1051
\@beginparpenalty -\@lowpenalty
\@endparpenalty -\@lowpenalty
\@itempenalty -\@lowpenalty
\binoppenalty=5000
\relpenalty=300
\clubpenalty=300
\widowpenalty=1000
\hyphenpenalty=15
\hfuzz=1pt
\emergencystretch=10pt
\thinmuskip=2.2mu
\medmuskip = 3.5mu plus 0.2mu minus .75mu
\thickmuskip = 5mu plus 3mu
\oddsidemargin 0.5in \evensidemargin 0.5in
 \topmargin 0pt \headheight 12pt \headsep 25pt \footskip 30pt
\textheight = 7.8in
\advance\textheight by \topskip
\textwidth 5.5in % changed from 5 in
\columnsep 10pt \columnseprule 0pt
\parskip 0pt plus 1.5pt
\parindent 1.5em
\topsep 10pt plus 4pt minus 6pt
\partopsep 3pt plus 2pt minus 2pt
\itemsep 5pt plus 2.5pt minus 1pt
\onecolumn}\makeatother

\message{setting values of counters}
\newcommand{\setpart}[1]{\setcounter{part}{#1}}
\newcommand{\setchap}[1]{\setcounter{chapter}{#1}}
\newcommand{\setsec}[1]{\setcounter{section}{#1}}
\newcommand{\setsubsec}[1]{\setcounter{subsection}{#1}}
\newcommand{\setpage}[1]{\setcounter{page}{#1}}
\typeout{End of arthead.tex}

